Demonstration Based Explainable AI for Learning from Demonstration Methods

Learning from Demonstration (LfD) is a powerful type of machine learning that can allow novices to teach and program robots to complete various tasks. However, the learning process for these systems may still be difficult for novices to interpret and understand, making effective teaching challenging. Explainable artificial intelligence (XAI) aims to address this challenge by explaining a system to the user. In this work, we investigate XAI within LfD by implementing an adaptive explanatory feedback system on an inverse reinforcement learning (IRL) algorithm. The feedback is implemented by demonstrating selected learnt trajectories to users. The system adapts to user teaching by categorizing and then selectively sampling trajectories shown to a user, to show a representative sample of both successful and unsuccessful trajectories. The system was evaluated through a user study with 26 participants teaching a robot a navigation task. The results of the user study demonstrated that the proposed explanatory feedback system can improve robot performance, teaching efficiency and user understanding of the robot.

==> figures/barplot_certainties.tex <==
\begin{tikzpicture}
    \definecolor{r}{RGB}{255,0,32}
    \definecolor{rw1}{RGB}{230, 50, 60}
    \definecolor{rw2}{RGB}{213, 123, 111}
    \definecolor{w}{RGB}{198, 198, 198}
    \definecolor{bw2}{RGB}{142, 160, 188}
    \definecolor{bw1}{RGB}{60, 130, 200}
    \definecolor{b}{RGB}{5,113,200}

    \pgfplotsset{
       /pgfplots/bar  cycle  list/.style={/pgfplots/cycle  list={%
            {r!75!black,fill=r!60!white,mark=none},%
            {rw1!75!black,fill=rw1!60!white,mark=none},%
            {rw2!75!black,fill=rw2!60!white,mark=none},%
            {w!75!black,fill=w!60!white,mark=none},%
            {bw2!75!black,fill=bw2!60!white,mark=none},%
            {bw1!75!black,fill=bw1!60!white,mark=none},%
            {b!75!black,fill=b!60!white,mark=none},%
         }
       },
    }
    
    \tikzstyle{every node}=[font=\small]

    
    
    
    \begin{axis}[
        % enlarge x limits=true,
        % enlarge y limits=true,
        name=mainplot,
        xbar stacked,
        title=\textbf{Initial Goal Predictions},
        nodes near coords,
        bar width=0.8,
        width = 0.36\textwidth,
        height = 0.18\textwidth,
        xmin = 0, xmax = 65,
        enlarge y limits={abs=10pt},
        ytick={2,1},
        yticklabels={F, NF},  
        xtick={0,13,26,39,52,65},
        xticklabels={0\%,20\%,40\%,60\%,80\%,100\%},         
        legend style={at={(0.5,-0.20)}, anchor=north, legend columns=-1, /tikz/every even column/.append style={column sep=0.5cm}},
        % cycle list name=black white
    ]
    
        \addplot coordinates
        {(0,2) (1,1)};
        
        \addplot coordinates
        {(5,2) (5,1)};
        
        \addplot coordinates
        {(11,2) (2,1)};
        
        \addplot coordinates
        {(7,2) (12,1)};
        
        \addplot coordinates
        {(18,2) (17,1)};
        
        \addplot coordinates
        {(13,2) (11,1)};  
        
        \addplot coordinates
        {(21,2) (17,1)};    
        
    \end{axis}
    \begin{axis}[
        % enlarge x limits=true,
        % enlarge y limits=true,
        name=secondplot,
        title=\textbf{Final Goal Predictions},
        at={(mainplot.north east)},
        xshift=0.75cm,
        anchor=north west,    
        xbar stacked,
        nodes near coords,
        bar width=0.8,
        width = 0.36\textwidth,
        height = 0.18\textwidth,
        xmin = 0, xmax = 65,
        enlarge y limits={abs=10pt},
        ytick={2,1},
        yticklabels={F, NF},  
        xtick={0,13,26,39,52,65},
        xticklabels={0\%,20\%,40\%,60\%,80\%,100\%},       
        legend style={at={(-0.1, -2.30)}, anchor=north, legend columns=-1, /tikz/every even column/.append style={column sep=0.5cm}},
        % cycle list name=black white
    ]
    
        \addplot coordinates
        {(0,2) (0,1)};
        
        \addplot coordinates
        {(0,2) (1,1)};
        
        \addplot coordinates
        {(3,2) (4,1)};
        
        \addplot coordinates
        {(3,2) (6,1)};
        
        \addplot coordinates
        {(5,2) (15,1)};
        
        \addplot coordinates
        {(7,2) (13,1)};  
        
        \addplot coordinates
        {(47,2) (26,1)};  
        
        \legend{1,2,3,4,5,6,7}
    \end{axis}
    \begin{axis}[
        % enlarge x limits=true,
        % enlarge y limits=true,
        name=thirdplot,
        title=\textbf{Initial Action Predictions},
        at={(mainplot.south west)},
        xshift=0cm,
        yshift=-1.3cm,
        anchor=north west,      
        xbar stacked,
        nodes near coords,
        bar width=0.8,
        width = 0.36\textwidth,
        height = 0.18\textwidth,
        xmin = 0, xmax = 65,
        enlarge y limits={abs=10pt},
        ytick={0,1,2.5},
        ytick={2,1},
        yticklabels={F, NF}, 
        xtick={0,13,26,39,52,65},
        xticklabels={0\%,20\%,40\%,60\%,80\%,100\%},        
        legend style={at={(0.5,-0.20)}, anchor=north, legend columns=-1, /tikz/every even column/.append style={column sep=0.5cm}},
        % cycle list name=black white
    ]
    
        \addplot coordinates
        {(0,2) (2,1)};
        
        \addplot coordinates
        {(6,2) (5,1)};
        
        \addplot coordinates
        {(3,2) (12,1)};
        
        \addplot coordinates
        {(11,2) (15,1)};
        
        \addplot coordinates
        {(24,2) (8,1)};
        
        \addplot coordinates
        {(13,2) (7,1)};  
        
        \addplot coordinates
        {(8,2) (16,1)};     
        
    \end{axis}
    \begin{axis}[
        % enlarge x limits=true,
        % enlarge y limits=true,
        name=fourthplot,
        title=\textbf{Final Action Predictions},
        at={(thirdplot.north east)},
        xshift=0.75cm,
        anchor=north west,      
        xbar stacked,
        nodes near coords,
        bar width=0.8,
        width = 0.36\textwidth,
        height = 0.18\textwidth,
        xmin = 0, xmax = 65,
        enlarge y limits={abs=10pt},
        ytick={0,1,2.5},
        ytick={2,1},
        yticklabels={F, NF}, 
        xtick={0,13,26,39,52,65},
        xticklabels={0\%,20\%,40\%,60\%,80\%,100\%},          
        legend style={at={(0.5,-0.20)}, anchor=north, legend columns=-1, /tikz/every even column/.append style={column sep=0.5cm}},
        % cycle list name=black white
    ]
    
        \addplot coordinates
        {(0,2) (0,1)};
        
        \addplot coordinates
        {(0,2) (0,1)};
        
        \addplot coordinates
        {(5,2) (0,1)};
        
        \addplot coordinates
        {(8,2) (10,1)};
        
        \addplot coordinates
        {(18,2) (17,1)};
        
        \addplot coordinates
        {(13,2) (19,1)};  
        
        \addplot coordinates
        {(21,2) (19,1)};     
        
    \end{axis}
    
\end{tikzpicture}

==> figures/barplot_only_understanding.tex <==
\begin{tikzpicture}
    \definecolor{r}{RGB}{255,0,32}
    \definecolor{rw1}{RGB}{230, 50, 60}
    \definecolor{rw2}{RGB}{213, 123, 111}
    \definecolor{w}{RGB}{198, 198, 198}
    \definecolor{bw2}{RGB}{142, 160, 188}
    \definecolor{bw1}{RGB}{60, 130, 200}
    \definecolor{b}{RGB}{5,113,200}

    \pgfplotsset{
       /pgfplots/bar  cycle  list/.style={/pgfplots/cycle  list={%
            {r!75!black,fill=r!60!white,mark=none},%
            {rw1!75!black,fill=rw1!60!white,mark=none},%
            {rw2!75!black,fill=rw2!60!white,mark=none},%
            {w!75!black,fill=w!60!white,mark=none},%
            {bw2!75!black,fill=bw2!60!white,mark=none},%
            {bw1!75!black,fill=bw1!60!white,mark=none},%
            {b!75!black,fill=b!60!white,mark=none},%
         }
       },
    }
    
    \tikzstyle{every node}=[font=\small]

    
    
    
    \begin{axis}[
        % enlarge x limits=true,
        % enlarge y limits=true,
        name=mainplot,
        xbar stacked,
        title=\textbf{Percieved Understanding},
        nodes near coords,
        bar width=0.8,
        width = 0.55\textwidth,
        height = 0.18\textwidth,
        xmin = 0, xmax = 16,
        enlarge y limits={abs=10pt},
        ytick={2,1},
        yticklabels={F, NF},  
        xtick={0,4,8,12,16},
        xticklabels={0\%,25\%,50\%,75\%,100\%},         
        legend style={at={(0.5,-0.3)}, anchor=north, legend columns=-1, /tikz/every even column/.append style={column sep=0.5cm}},
        % cycle list name=black white
    ]
    
        \addplot coordinates
        {(0,2) (2,1)};
        
        \addplot coordinates
        {(0,2) (0,1)};
        
        \addplot coordinates
        {(1,2) (3,1)};
        
        \addplot coordinates
        {(2,2) (1,1)};
        
        \addplot coordinates
        {(6,2) (3,1)};
        
        \addplot coordinates
        {(4,2) (5,1)};  
        
        \addplot coordinates
        {(3,2) (2,1)};  
        
        \legend{St.D, D, Sl.D, N, Sl.A, A, St.A}
    \end{axis}
    % \begin{axis}[
    %     % enlarge x limits=true,
    %     % enlarge y limits=true,
    %     name=secondplot,
    %     title=\textbf{Q2: Understanding},
    %     at={(mainplot.north east)},
    %     xshift=0.75cm,
    %     anchor=north west,    
    %     xbar stacked,
    %     nodes near coords,
    %     bar width=0.8,
    %     width = 0.36\textwidth,
    %     height = 0.18\textwidth,
    %     xmin = 0, xmax = 16,
    %     enlarge y limits={abs=10pt},
    %     ytick={2,1},
    %     yticklabels={,},  
    %     xtick={0,4,8,12,16},
    %     xticklabels={0\%,25\%,50\%,75\%,100\%},         
    %     legend style={at={(-0.1, -2.30)}, anchor=north, legend columns=-1, /tikz/every even column/.append style={column sep=0.5cm}},
    %     % cycle list name=black white
    % ]
    
    %     \addplot coordinates
    %     {(0,2) (2,1)};
        
    %     \addplot coordinates
    %     {(0,2) (0,1)};
        
    %     \addplot coordinates
    %     {(1,2) (3,1)};
        
    %     \addplot coordinates
    %     {(2,2) (1,1)};
        
    %     \addplot coordinates
    %     {(6,2) (3,1)};
        
    %     \addplot coordinates
    %     {(4,2) (5,1)};  
        
    %     \addplot coordinates
    %     {(3,2) (2,1)};  
        
    %     \legend{St.D, D, Sl.D, N, Sl.A, A, St.A}
    % \end{axis}
    % \begin{axis}[
    %     % enlarge x limits=true,
    %     % enlarge y limits=true,
    %     name=thirdplot,
    %     title=\textbf{Q3: Teaching},
    %     at={(mainplot.south west)},
    %     xshift=0cm,
    %     yshift=-1.3cm,
    %     anchor=north west,      
    %     xbar stacked,
    %     nodes near coords,
    %     bar width=0.8,
    %     width = 0.36\textwidth,
    %     height = 0.18\textwidth,
    %     xmin = 0, xmax = 16,
    %     enlarge y limits={abs=10pt},
    %     ytick={0,1,2.5},
    %     ytick={2,1},
    %     yticklabels={,},  
    %     xtick={0,4,8,12,16},
    %     xticklabels={0\%,25\%,50\%,75\%,100\%},         
    %     legend style={at={(0.5,-0.20)}, anchor=north, legend columns=-1, /tikz/every even column/.append style={column sep=0.5cm}},
    %     % cycle list name=black white
    % ]
    
    %     \addplot coordinates
    %     {(0,2) (1,1)};
        
    %     \addplot coordinates
    %     {(1,2) (2,1)};
        
    %     \addplot coordinates
    %     {(1,2) (2,1)};
        
    %     \addplot coordinates
    %     {(1,2) (5,1)};
        
    %     \addplot coordinates
    %     {(10,2) (1,1)};
        
    %     \addplot coordinates
    %     {(3,2) (3,1)};  
        
    %     \addplot coordinates
    %     {(0,2) (2,1)};     
        
    % \end{axis}
    % \begin{axis}[
    %     % enlarge x limits=true,
    %     % enlarge y limits=true,
    %     name=fourthplot,
    %     title=\textbf{Q4: Mental Demand},
    %     at={(thirdplot.north east)},
    %     xshift=0.75cm,
    %     anchor=north west,      
    %     xbar stacked,
    %     nodes near coords,
    %     bar width=0.8,
    %     width = 0.36\textwidth,
    %     height = 0.18\textwidth,
    %     xmin = 0, xmax = 16,
    %     enlarge y limits={abs=10pt},
    %     ytick={0,1,2.5},
    %     ytick={2,1},
    %     yticklabels={,},  
    %     xtick={0,4,8,12,16},
    %     xticklabels={0\%,25\%,50\%,75\%,100\%},         
    %     legend style={at={(0.5,-0.20)}, anchor=north, legend columns=-1, /tikz/every even column/.append style={column sep=0.5cm}},
    %     % cycle list name=black white
    % ]
    
    %     \addplot coordinates
    %     {(0,2) (1,1)};
        
    %     \addplot coordinates
    %     {(1,2) (2,1)};
        
    %     \addplot coordinates
    %     {(1,2) (2,1)};
        
    %     \addplot coordinates
    %     {(1,2) (5,1)};
        
    %     \addplot coordinates
    %     {(10,2) (1,1)};
        
    %     \addplot coordinates
    %     {(3,2) (3,1)};  
        
    %     \addplot coordinates
    %     {(0,2) (2,1)};     
        
    % \end{axis}
    
\end{tikzpicture}

==> figures/barplot_second_study.tex <==
\begin{tikzpicture}
    \definecolor{r}{RGB}{255,0,32}
    \definecolor{rw1}{RGB}{230, 50, 60}
    \definecolor{rw2}{RGB}{213, 123, 111}
    \definecolor{w}{RGB}{198, 198, 198}
    \definecolor{bw2}{RGB}{142, 160, 188}
    \definecolor{bw1}{RGB}{60, 130, 200}
    \definecolor{b}{RGB}{5,113,200}

    \pgfplotsset{
       /pgfplots/bar  cycle  list/.style={/pgfplots/cycle  list={%
            {r!75!black,fill=r!60!white,mark=none},%
            {rw1!75!black,fill=rw1!60!white,mark=none},%
            {rw2!75!black,fill=rw2!60!white,mark=none},%
            {w!75!black,fill=w!60!white,mark=none},%
            {bw2!75!black,fill=bw2!60!white,mark=none},%
            {bw1!75!black,fill=bw1!60!white,mark=none},%
            {b!75!black,fill=b!60!white,mark=none},%
         }
       },
    }
    
    \tikzstyle{every node}=[font=\small]

    
    
    
    \begin{axis}[
        % enlarge x limits=true,
        % enlarge y limits=true,
        name=mainplot,
        xbar stacked,
        title=\textbf{Q1: Robot Satisfaction},
        nodes near coords,
        bar width=0.8,
        width = 0.36\textwidth,
        height = 0.18\textwidth,
        xmin = 0, xmax = 16,
        enlarge y limits={abs=10pt},
        ytick={2,1},
        yticklabels={F, NF},  
        xtick={0,4,8,12,16},
        xticklabels={0\%,25\%,50\%,75\%,100\%},         
        legend style={at={(0.5,-0.20)}, anchor=north, legend columns=-1, /tikz/every even column/.append style={column sep=0.5cm}},
        % cycle list name=black white
    ]
    
        \addplot coordinates
        {(1,2) (2,1)};
        
        \addplot coordinates
        {(1,2) (0,1)};
        
        \addplot coordinates
        {(3,2) (1,1)};
        
        \addplot coordinates
        {(0,2) (3,1)};
        
        \addplot coordinates
        {(6,2) (6,1)};
        
        \addplot coordinates
        {(5,2) (1,1)};  
        
        \addplot coordinates
        {(0,2) (3,1)};    
        
    \end{axis}
    \begin{axis}[
        % enlarge x limits=true,
        % enlarge y limits=true,
        name=secondplot,
        title=\textbf{Q2: Understanding},
        at={(mainplot.north east)},
        xshift=0.75cm,
        anchor=north west,    
        xbar stacked,
        nodes near coords,
        bar width=0.8,
        width = 0.36\textwidth,
        height = 0.18\textwidth,
        xmin = 0, xmax = 16,
        enlarge y limits={abs=10pt},
        ytick={2,1},
        yticklabels={,},  
        xtick={0,4,8,12,16},
        xticklabels={0\%,25\%,50\%,75\%,100\%},         
        legend style={at={(-0.1, -2.30)}, anchor=north, legend columns=-1, /tikz/every even column/.append style={column sep=0.5cm}},
        % cycle list name=black white
    ]
    
        \addplot coordinates
        {(0,2) (2,1)};
        
        \addplot coordinates
        {(0,2) (0,1)};
        
        \addplot coordinates
        {(1,2) (3,1)};
        
        \addplot coordinates
        {(2,2) (1,1)};
        
        \addplot coordinates
        {(6,2) (3,1)};
        
        \addplot coordinates
        {(4,2) (5,1)};  
        
        \addplot coordinates
        {(3,2) (2,1)};  
        
        \legend{St.D, D, Sl.D, N, Sl.A, A, St.A}
    \end{axis}
    \begin{axis}[
        % enlarge x limits=true,
        % enlarge y limits=true,
        name=thirdplot,
        title=\textbf{Q3: Teaching},
        at={(mainplot.south west)},
        xshift=0cm,
        yshift=-1.3cm,
        anchor=north west,      
        xbar stacked,
        nodes near coords,
        bar width=0.8,
        width = 0.36\textwidth,
        height = 0.18\textwidth,
        xmin = 0, xmax = 16,
        enlarge y limits={abs=10pt},
        ytick={0,1,2.5},
        ytick={2,1},
        yticklabels={,},  
        xtick={0,4,8,12,16},
        xticklabels={0\%,25\%,50\%,75\%,100\%},         
        legend style={at={(0.5,-0.20)}, anchor=north, legend columns=-1, /tikz/every even column/.append style={column sep=0.5cm}},
        % cycle list name=black white
    ]
    
        \addplot coordinates
        {(0,2) (1,1)};
        
        \addplot coordinates
        {(1,2) (2,1)};
        
        \addplot coordinates
        {(1,2) (2,1)};
        
        \addplot coordinates
        {(1,2) (5,1)};
        
        \addplot coordinates
        {(10,2) (1,1)};
        
        \addplot coordinates
        {(3,2) (3,1)};  
        
        \addplot coordinates
        {(0,2) (2,1)};     
        
    \end{axis}
    \begin{axis}[
        % enlarge x limits=true,
        % enlarge y limits=true,
        name=fourthplot,
        title=\textbf{Q4: Mental Demand},
        at={(thirdplot.north east)},
        xshift=0.75cm,
        anchor=north west,      
        xbar stacked,
        nodes near coords,
        bar width=0.8,
        width = 0.36\textwidth,
        height = 0.18\textwidth,
        xmin = 0, xmax = 16,
        enlarge y limits={abs=10pt},
        ytick={0,1,2.5},
        ytick={2,1},
        yticklabels={,},  
        xtick={0,4,8,12,16},
        xticklabels={0\%,25\%,50\%,75\%,100\%},         
        legend style={at={(0.5,-0.20)}, anchor=north, legend columns=-1, /tikz/every even column/.append style={column sep=0.5cm}},
        % cycle list name=black white
    ]
    
        \addplot coordinates
        {(0,2) (1,1)};
        
        \addplot coordinates
        {(1,2) (2,1)};
        
        \addplot coordinates
        {(1,2) (2,1)};
        
        \addplot coordinates
        {(1,2) (5,1)};
        
        \addplot coordinates
        {(10,2) (1,1)};
        
        \addplot coordinates
        {(3,2) (3,1)};  
        
        \addplot coordinates
        {(0,2) (2,1)};     
        
    \end{axis}
    
\end{tikzpicture}

==> figures/barplot_third_study.tex <==
\begin{tikzpicture}
    \definecolor{r}{RGB}{255,0,32}
    \definecolor{rw1}{RGB}{230, 50, 60}
    \definecolor{rw2}{RGB}{213, 123, 111}
    \definecolor{w}{RGB}{198, 198, 198}
    \definecolor{bw2}{RGB}{142, 160, 188}
    \definecolor{bw1}{RGB}{60, 130, 200}
    \definecolor{b}{RGB}{5,113,200}

    \pgfplotsset{
       /pgfplots/bar  cycle  list/.style={/pgfplots/cycle  list={%
            {r!75!black,fill=r!60!white,mark=none},%
            {rw1!75!black,fill=rw1!60!white,mark=none},%
            {rw2!75!black,fill=rw2!60!white,mark=none},%
            {w!75!black,fill=w!60!white,mark=none},%
            {bw2!75!black,fill=bw2!60!white,mark=none},%
            {bw1!75!black,fill=bw1!60!white,mark=none},%
            {b!75!black,fill=b!60!white,mark=none},%
         }
       },
    }
    
    \tikzstyle{every node}=[font=\small]

    
    
    
    \begin{axis}[
        % enlarge x limits=true,
        % enlarge y limits=true,
        name=mainplot,
        xbar stacked,
        title=\textbf{Q1: Robot Satisfaction},
        nodes near coords,
        bar width=0.8,
        width = 0.36\textwidth,
        height = 0.18\textwidth,
        xmin = 0, xmax = 13,
        enlarge y limits={abs=10pt},
        ytick={2,1},
        yticklabels={IF, PF},  
        xtick={0,4,8,12,16},
        xticklabels={0\%,25\%,50\%,75\%,100\%},         
        legend style={at={(0.5,-0.20)}, anchor=north, legend columns=-1, /tikz/every even column/.append style={column sep=0.5cm}},
        % cycle list name=black white
    ]
    
        \addplot coordinates
        {(0,2) (0,1)};
        
        \addplot coordinates
        {(0,2) (0,1)};
        
        \addplot coordinates
        {(0,2) (1,1)};
        
        \addplot coordinates
        {(2,2) (0,1)};
        
        \addplot coordinates
        {(3,2) (4,1)};
        
        \addplot coordinates
        {(6,2) (6,1)};  
        
        \addplot coordinates
        {(2,2) (2,1)};    
        
    \end{axis}
    \begin{axis}[
        % enlarge x limits=true,
        % enlarge y limits=true,
        name=secondplot,
        title=\textbf{Q2: Perceived Understanding},
        at={(mainplot.north east)},
        xshift=0.75cm,
        anchor=north west,    
        xbar stacked,
        nodes near coords,
        bar width=0.8,
        width = 0.36\textwidth,
        height = 0.18\textwidth,
        xmin = 0, xmax = 13,
        enlarge y limits={abs=10pt},
        ytick={2,1},
        yticklabels={IF, PF},  
        xtick={0,4,8,12,16},
        xticklabels={0\%,25\%,50\%,75\%,100\%},         
        legend style={at={(-0.1, -2.30)}, anchor=north, legend columns=-1, /tikz/every even column/.append style={column sep=0.5cm}},
        % cycle list name=black white
    ]
    
        \addplot coordinates
        {(0,2) (0,1)};
        
        \addplot coordinates
        {(0,2) (0,1)};
        
        \addplot coordinates
        {(1,2) (0,1)};
        
        \addplot coordinates
        {(0,2) (1,1)};
        
        \addplot coordinates
        {(3,2) (5,1)};
        
        \addplot coordinates
        {(6,2) (6,1)};  
        
        \addplot coordinates
        {(3,2) (1,1)};  
        
        \legend{St.D, D, Sl.D, N, Sl.A, A, St.A}
    \end{axis}
    \begin{axis}[
        % enlarge x limits=true,
        % enlarge y limits=true,
        name=thirdplot,
        title=\textbf{Q3: Teaching},
        at={(mainplot.south west)},
        xshift=0cm,
        yshift=-1.3cm,
        anchor=north west,      
        xbar stacked,
        nodes near coords,
        bar width=0.8,
        width = 0.36\textwidth,
        height = 0.18\textwidth,
        xmin = 0, xmax = 13,
        enlarge y limits={abs=10pt},
        ytick={0,1,2.5},
        ytick={2,1},
        yticklabels={IF, PF}, 
        xtick={0,4,8,12,16},
        xticklabels={0\%,25\%,50\%,75\%,100\%},         
        legend style={at={(0.5,-0.20)}, anchor=north, legend columns=-1, /tikz/every even column/.append style={column sep=0.5cm}},
        % cycle list name=black white
    ]
    
        \addplot coordinates
        {(0,2) (0,1)};
        
        \addplot coordinates
        {(1,2) (0,1)};
        
        \addplot coordinates
        {(1,2) (4,1)};
        
        \addplot coordinates
        {(0,2) (1,1)};
        
        \addplot coordinates
        {(6,2) (6,1)};
        
        \addplot coordinates
        {(3,2) (2,1)};  
        
        \addplot coordinates
        {(2,2) (0,1)};     
        
    \end{axis}
    \begin{axis}[
        % enlarge x limits=true,
        % enlarge y limits=true,
        name=fourthplot,
        title=\textbf{Q4: Mental Demand},
        at={(thirdplot.north east)},
        xshift=0.75cm,
        anchor=north west,      
        xbar stacked,
        nodes near coords,
        bar width=0.8,
        width = 0.36\textwidth,
        height = 0.18\textwidth,
        xmin = 0, xmax = 13,
        enlarge y limits={abs=10pt},
        ytick={0,1,2.5},
        ytick={2,1},
        yticklabels={IF, PF}, 
        xtick={0,4,8,12,16},
        xticklabels={0\%,25\%,50\%,75\%,100\%},         
        legend style={at={(0.5,-0.20)}, anchor=north, legend columns=-1, /tikz/every even column/.append style={column sep=0.5cm}},
        % cycle list name=black white
    ]
    
        \addplot coordinates
        {(2,2) (0,1)};
        
        \addplot coordinates
        {(2,2) (6,1)};
        
        \addplot coordinates
        {(5,2) (3,1)};
        
        \addplot coordinates
        {(2,2) (1,1)};
        
        \addplot coordinates
        {(1,2) (2,1)};
        
        \addplot coordinates
        {(0,2) (1,1)};  
        
        \addplot coordinates
        {(1,2) (0,1)};     
        
    \end{axis}
    
\end{tikzpicture}
